Formalization of Fragments of the Theory of Hereditarily Finite Sets

The axiomatization of the theory of hereditarily finite sets in first-order classical logic is systematically explored and formalized in Isabelle/HOL. The formalization uses a hierarchy of locales, each corresponding to a fragment of the theory given by a particular collection of axioms. An inductive definition of first-order definable predicates is introduced and used to formalize axiom schemata. Special attention is paid to several equivalent axioms of finiteness, as well as to several equivalent ways of expressing regularity. The work also formalizes several facts about the independence of an axiom from a system of axioms by defining appropriate models.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Mircea Marin, Adrian Cr\u{a}ciun (Eds.): FROM 2026\\
EPTCS 452, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.452.1}{10.4204/EPTCS.452.1}}

